UniT: Unified Multimodal Chain-of-Thought Test-time Scaling

Unified models can handle both multimodal understanding and generation within a single architecture, yet they typically operate in a single pass without iteratively refining their outputs. Many multimodal tasks, especially those involving complex spatial compositions, multiple interacting objects, or evolving instructions, require decomposing instructions, verifying intermediate results, and making iterative corrections. While test-time scaling (TTS) has demonstrated that allocating additional inference compute for iterative reasoning substantially improves language model performance, extending this paradigm to unified multimodal models remains an open challenge. We introduce UniT, a framework for multimodal chain-of-thought test-time scaling that enables a single unified model to reason, verify, and refine across multiple rounds. UniT combines agentic data synthesis, unified model training, and flexible test-time inference to elicit cognitive behaviors including verification, subgoal decomposition, and content memory. Our key findings are: (1) unified models trained on short reasoning trajectories generalize to longer inference chains at test time; (2) sequential chain-of-thought reasoning provides a more scalable and compute-efficient TTS strategy than parallel sampling; (3) training on generation and editing trajectories improves out-of-distribution visual reasoning. These results establish multimodal test-time scaling as an effective paradigm for advancing both generation and understanding in unified models.

==> preamble.tex <==
% Legacy preamble retained for compatibility.



==> sec/0_abstract.tex <==
\begin{abstract}
Unified models can handle both multimodal understanding and generation within a single architecture, yet they typically operate in a single pass without iteratively refining their outputs. Many multimodal tasks, especially those involving complex spatial compositions, multiple interacting objects, or evolving instructions, require decomposing instructions, verifying intermediate results, and making iterative corrections. While test-time scaling (TTS) has demonstrated that allocating additional inference compute for iterative reasoning substantially improves language model performance, extending this paradigm to unified multimodal models remains an open challenge.

We introduce \methodname, a framework for multimodal chain-of-thought test-time scaling that enables a single unified model to reason, verify, and refine across multiple rounds. \methodname~combines agentic data synthesis, unified model training, and flexible test-time inference to elicit cognitive behaviors including verification, subgoal decomposition, and content memory. Our key findings are: (1) unified models trained on short reasoning trajectories generalize to longer inference chains at test time; (2) sequential chain-of-thought reasoning provides a more scalable and compute-efficient TTS strategy than parallel sampling; (3) training on generation and editing trajectories improves out-of-distribution visual reasoning. These results establish multimodal test-time scaling as an effective paradigm for advancing both generation and understanding in unified models.
\end{abstract}


==> sec/0_abstract_improved.tex <==
\begin{abstract}
Unified models can handle both multimodal understanding and generation within a single architecture, yet they typically operate in a single pass without iteratively refining their outputs. Many multimodal tasks—especially those involving complex spatial compositions, multiple interacting objects, or evolving instructions—require decomposing instructions, verifying intermediate results, and making iterative corrections. While test-time scaling (TTS) has demonstrated that allocating additional inference compute for iterative reasoning substantially improves language model performance, extending this paradigm to unified multimodal models remains an open challenge.

We introduce \methodname, a framework for multimodal chain-of-thought test-time scaling that enables a single unified model to reason, verify, and refine across multiple rounds. \methodname~combines agentic data synthesis, unified model training, and flexible test-time inference to elicit cognitive behaviors including verification, subgoal decomposition, and content memory. Our key findings are: (1) unified models trained on short reasoning trajectories generalize to longer inference chains at test time; (2) sequential chain-of-thought reasoning provides a more scalable and compute-efficient TTS strategy than parallel sampling; (3) training on generation and editing trajectories improves out-of-distribution visual reasoning. These results establish multimodal test-time scaling as an effective paradigm for advancing both generation and understanding in unified models.
\end{abstract}


==> sec/0_abstract_ziqi_version.tex <==
\begin{abstract}
Unified models hold the promise of handling multimodal understanding and generation within a single architecture, yet they largely operate in a single-pass manner without iteratively reconsidering or refining their outputs. Many multimodal tasks, especially those involving complex spatial compositions, multiple interacting objects, or complex evolving instructions, naturally require inspecting intermediate results, identifying inconsistencies, and making iterative corrections. On the other hand, Test-time scaling (TTS) in language models has shown that allocating additional inference compute for such iterative reasoning can substantially improve performance, but how to extend this paradigm to unified multimodal models remains an open question.

To bridge this gap, we propose \methodname, a framework for multimodal chain-of-thought test-time scaling that equips a single unified model with the ability to reason, verify, and refine across multiple rounds. \methodname  ~combines agentic data synthesis, unified model training, and flexible test-time inference to induce multimodal cognitive behaviors such as verification, subgoal decomposition, and content memory. Our key insights are: (1) unified models trained on short reasoning trajectories can naturally extrapolate to longer inference chains when given more compute, and (2) sequential chain-of-thought refinement provides a more compute-efficient strategy than parallel sampling. These findings position multimodal test-time scaling as a general and effective paradigm for improving both generation and comprehension in unified models.
\end{abstract}


==> sec/1_intro_ziqi_version.tex <==
\section{Introduction}
\label{sec:intro}

% Unified multimodal models~\citep{deng2025emerging,wu2025janus,zhou2024transfusion} aim to merge vision, language, and other modalities into a single architecture capable of understanding and generation. Compared with modular pipelines, these models promise seamless cross-modal grounding, interleaved reasoning, and end-to-end adaptability, which are essential for building general-purpose multimodal assistants. However, despite their expressive capacity, current unified models operate mostly in a single-pass inference mode: they produce an output once, without evaluating, reflecting, or refining their own predictions. This limitation becomes fundamental in settings like compositional synthesis or editing, and complex visual reasoning, which require multi-step reasoning, contextual coherence across rounds, or iterative improvement through self-correction.
% Unified multimodal models~\citep{deng2025emerging,wu2025janus,zhou2024transfusion} aim to merge vision, language, and other modalities into a single architecture capable of both understanding and generation. Unlike modular pipelines, where separate models handle perception, verification, and synthesis, a unified model maintains all modalities within one coherent conversation. This enables richer cross-modal grounding, continuous contextual tracking, and seamless interleaving of understanding and generation. Such properties make unified models potentially promising for tasks where instructions are complex or could evolve over time, where multiple visual elements interact, or where outputs could be iteratively refined. However, existing unified models still operate mostly in a \emph{single-pass} mode: they produce an output once, without explicit designs in evaluating, reflecting on, or refining their predictions. This stands in contrast to tasks that intrinsically require multi-step reasoning and self-correction, such as compositional synthesis, iterative editing, and complex visual reasoning, where both humans and models naturally benefit from iterative inspection and refinement.

Unified multimodal models~\citep{deng2025emerging,wu2025janus,zhou2024transfusion} aim to merge vision, language, and other modalities into a single architecture capable of both understanding and generation. Unlike modular pipelines, where separate models handle perception, verification, and synthesis, a unified model maintains all modalities within one coherent round. This enables richer cross-modal grounding, continuous contextual tracking, and seamless interleaving of understanding and generation. Such properties make unified models naturally suited for tasks where multiple multimodal elements interact, where outputs benefit from iterative refinement, or where instructions are complex or evolve over time.
However, despite this potential, existing unified models still operate mostly in a \emph{single-pass} mode: they produce an output once, without explicit mechanisms for evaluating, reflecting on, or refining their predictions. This stands in contrast to tasks that intrinsically require multi-step reasoning and self-correction, such as compositional synthesis, iterative editing, and complex visual reasoning - settings where both humans and models naturally benefit from iterative inspection and refinement.



In parallel, the large language model (LLM) community have shown that test-time scaling (TTS) - allocating additional inference compute via extended chain-of-thought reasoning, verification, and iterative refinement~\citep{jaech2024openai,guo2025deepseek,snell2024scaling} - yields substantial gains in tasks involving mathematics~\citep{cobbe2021training}, code generation~\citep{chen2021evaluating}, and complex logical reasoning~\citep{srivastava2023beyond}. Early work on multimodal chain-of-thought has demonstrated similar benefits for single-round visual understanding and simple generation~\citep{visualcot,fang2025got,xiao2025mindomni,interleaving-reasoning,chern2025thinking}. Yet, scalable test-time reasoning for unified multimodal models remains essentially unexplored. Unified models lack both the training data and mechanisms required to support iterative multimodal computation, or reasoning over visual and textual context, verifying outputs, and refining images. Bridging this gap requires a framework that can systematically integrate data creation, unified model training, and flexible test-time inference together. This motivates the central question of this work:
\textbf{\textit{How to enable scalable multimodal inference that allows unified models to iteratively generate, reflect, and refine?}}



To this end, we propose \textbf{\textit{UniT}}, a comprehensive framework for unified multimodal chain-of-thought test-time scaling. Our key insight is that scalable multimodal inference requires the tight integration of three components: \textbf{\textit{1) Agentic data synthesis.}}
We construct multi-round trajectories where a vision-language agent critiques, verifies, and decomposes tasks, while an image-editing model iteratively refines outputs. This produces training data with explicit multimodal chain-of-thought and three core cognitive behaviors:
verification, subgoal decomposition, and content memory. \textbf{\textit{2) Unified multimodal model training.}}
These trajectories are used to fine-tune a unified model (Bagel~\citep{deng2025emerging}), enabling it to internalize multimodal reasoning patterns and perform both understanding and refinement without switching models. \textbf{\textit{3) Multimodal test-time scaling.}}
At inference, the model receives a flexible computational budget and performs iterative reasoning and refinement in a fully self-contained manner, allocating more rounds to more challenging tasks.


The synergy of these components enables the model to act as a single, coherent multimodal reasoner capable of self-evaluation and iterative improvement. Our automated pipeline yields approximately 12k multi-round trajectories (average 3.6 refinement steps), leading to a unified model that performs reasoning, verification, and image editing internally through explicit multimodal chain-of-thought. Despite being trained on short trajectories, the unified model naturally extrapolates to longer inference chains (averaging 4.7 rounds), echoing patterns previously seen only in text-only models~\citep{snell2024scaling}. Moreover, sequential chain-of-thought scaling significantly outperforms best-of-N parallel sampling, achieving comparable performance using 2.5× less compute. These results indicate that iterative refinement with explicit reasoning is a more compute-efficient strategy for multimodal generation. UniT delivers substantial improvements across diverse domains such as image generation, compositional editing, multi-turn editing, and visual reasoning.

We summarize our contributions as follows:
\begin{itemize}
    \item \textbf{Unified multimodal test-time scaling.} We propose \textbf{UniT}, the first unified framework for multimodal chain-of-thought test-time scaling, integrating agentic data synthesis, unified multimodal training, and iterative inference.
    \item \textbf{Emergent extrapolation to longer reasoning chains.} We show that unified models trained on short reasoning trajectories generalize to longer inference chains at test time, revealing emergent multimodal test-time scaling.
    \item \textbf{Broad improvements across multimodal tasks.} UniT achieves substantial gains on compositional generation, multi-turn editing, and visual reasoning benchmarks, demonstrating chain-of-thought test-time scaling as an effective and general paradigm for multimodal intelligence.
\end{itemize}

